xView3-SAR: Detecting Dark Fishing Activity Using Synthetic Aperture Radar Imagery

Unsustainable fishing practices worldwide pose a major threat to marine resources and ecosystems. Identifying vessels that do not show up in conventional monitoring systems -- known as ``dark vessels'' -- is key to managing and securing the health of marine environments. With the rise of satellite-based synthetic aperture radar (SAR) imaging and modern machine learning (ML), it is now possible to automate detection of dark vessels day or night, under all-weather conditions. SAR images, however, require a domain-specific treatment and are not widely accessible to the ML community. Maritime objects (vessels and offshore infrastructure) are relatively small and sparse, challenging traditional computer vision approaches. We present the largest labeled dataset for training ML models to detect and characterize vessels and ocean structures in SAR imagery. xView3-SAR consists of nearly 1,000 analysis-ready SAR images from the Sentinel-1 mission that are, on average, 29,400-by-24,400 pixels each. The images are annotated using a combination of automated and manual analysis. Co-located bathymetry and wind state rasters accompany every SAR image. We also provide an overview of the xView3 Computer Vision Challenge, an international competition using xView3-SAR for ship detection and characterization at large scale. We release the data (\href{https://iuu.xview.us/}{https://iuu.xview.us/}) and code (\href{https://github.com/DIUx-xView}{https://github.com/DIUx-xView}) to support ongoing development and evaluation of ML approaches for this important application.

==> sec/11_checklist.tex <==
\appendix

% --- PDF will be split by an editor (e.g. macOS preview), so need to restart from page 1
\setcounter{page}{1}

% --- repeat the title (AT: haven't found a more elegant way to do this...)
\onecolumn
%
\begin{center}
{\large
\textbf{xView3-SAR: Detecting Dark Fishing Activity Using Synthetic Aperture Radar Imagery}} \\

\vspace{1em}
Paper Checklist
\end{center}

\vspace{2em}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
    \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? \textcolor{blue}{[YES]} We created and evaluated a dataset for the detection of IUU fishing from Sentinel-1 synthetic aperture radar imagery. The construction of the dataset can be understood in Section \ref{sec:dataset} and additional information can be found in the Supplementary Material.
    \item Have you read the ethics review guidelines and ensured that your paper conforms to them? \textcolor{blue}{[YES]}
    \item Did you discuss any potential negative societal impacts of your work? \textcolor{gray}{[N/A]}
    \item Did you describe the limitations of your work? \textcolor{blue}{[YES]} We provide a discussion of the limitations of geographic coverage in Section \ref{sec:dataset}. Section \ref{sec:conclusion} discusses the mediocre performance of the models for close-to-shore vessels. Lastly, we provide a thorough analysis of the precision, recall, and F1 scores of the winning model in Appendix Section \ref{sec:appendix:winning-model-perf}, highlighting areas where the models and/or data sources need to be improved.
\end{enumerate}

\item If you are including theoretical results… \textcolor{gray}{[N/A]}

\item{If you ran experiments...}
\begin{enumerate}
    \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? \textcolor{blue}{[YES]} The link to source code is provided in the body of the paper as well as in the Supplementary Material. All source code for reference and winning models, Dockerized containers for the models, and detailed documentation is available at \href{https://github.com/DIUx-xView/}{https://github.com/DIUx-xView/} in each model’s respective repositories.
    \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? \textcolor{blue}{[YES]} Similarly to the answer above, all details are available publicly at the link above in the proper repository for each model.
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? \textcolor{gray}{[N/A]}
    \item Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? \textcolor{blue}{[YES]} Each model provides these details in the repositories at the link above.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
    \item If your work uses existing assets, did you cite the creators? \textcolor{blue}{[YES]} The Sentinel-1 data we use is properly cited, and work from competitors is properly attributed.
    \item Did you mention the license of the assets? \textcolor{blue}{[YES]} The dataset is licensed CC NC-BY-SA 4.0. All models are licensed as Apache 2.0, BSD, LGPL, or MIT.
    \item Did you include any new assets either in the supplemental material or as a URL? \textcolor{red}{[No]}
    \item Did you discuss whether and how consent was obtained from people whose data you're using/curating? \textcolor{gray}{[N/A]}
    \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content? \textcolor{gray}{[N/A]} The Sentinel-1 satellite data is too steep of a graze angle (almost vertical) and too low resolution (~10m GSD) to contain any personally identifiable information.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
    \item Did you include the full text of instructions given to participants and screenshots, if applicable? \textcolor{blue}{[YES]} For the subset of labels that were manually annotated, the instructions are provided as-is (with minor TeX edits) in Supplemental Material Section \ref{sec:appendix:labeling_instructions}.
    \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable? \textcolor{gray}{[N/A]}
    \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation? \textcolor{gray}{[N/A]}
\end{enumerate}

\end{enumerate}

==> sec/12_datasheet.tex <==
\appendix

% --- PDF will be split by an editor (e.g. macOS preview), so need to restart from page 1
\setcounter{page}{1}

% --- repeat the title (AT: haven't found a more elegant way to do this...)
\onecolumn
%
\begin{center}
{\large
\textbf{xView3-SAR: Detecting Dark Fishing Activity Using Synthetic Aperture Radar Imagery}} \\

\vspace{1em}
Datasheet and Documentation
\end{center}

\vspace{2em}

\begin{enumerate}[label=\textbf{Q{\arabic*}}]
    \item \textbf{What do the instances that comprise the dataset represent (e.g., documents, photos, people, countries)?} \vspace{3pt}

    % \begin{enumerate}
        % \item
        Each dataset instance consists of a set of input rasters $X_i$ and a set of output labels $Y_i$. Each $X_i$ is comprised of:
        \begin{itemize}
            \item VH\_dB.tif: VH-polarization SAR image (dB), 10-meter pixels
            \item VV\_dB.tif: VV-polarization SAR image (dB), 10-meter pixels
            \item bathymetry.tif: bathymetry and elevation image (meters), 500-meter pixels
            \item owiWindSpeed.tif: wind speed (meters per second), 500-meter pixels
            \item owiWindDirection.tif: wind direction (degrees clockwise from north), 500-meter pixels
            \item owiWindQuality.tif: wind quality mask (0 good, 1 medium, 2 low, 3 or), 500-meter pixels
            \item owiMask.tif: land/ice mask (0 valid, 1 land, 2 ice), 500-meter pixels
        \end{itemize}
        Each $Y_i$ is comprised of multiple data fields described further below.
    % \end{enumerate}
    \item \textbf{How many instances are there in total (of each type, if appropriate)?} \vspace{3pt}
    
    % \begin{enumerate}
        % \item A: 
    There are 991 sets of input rasters and 243,018 associated labels.
    % \end{enumerate}
    \item \textbf{Does the dataset contain all possible instances or is it a sample (not necessarily random) of instances from a larger set?}  \vspace{3pt}
    
    % \begin{enumerate}
        % \item A: 
    The dataset contains strategically chosen regions across the world that are known for: (1) high incidences of AIS usage which provide an abundant source of high-confidence, matched labels; (2) high incidences of IUU fishing; (3) high incidences of fixed infrastructure. %This choice imparts a specific distribution on the data and may not be representative of all regions of the world.
        
    Of the chosen regions, we included images that contain a large variety of object types (vessel and non-vessel) and vessel sizes and types. % As such, there is a healthy range in distribution of vessel types, sizes, and patterns within the dataset.
        
    The design decisions reflect the objective of this dataset---characterizing maritime objects to aid anti-IUU fishing missions.
    % \end{enumerate}
    \item \textbf{What data does each instance consist of?} \vspace{3pt}
    
    % \begin{enumerate}
        % \item A: 
    A label file is provided as a CSV containing the following columns corresponding to label fields:
        \begin{itemize}
            \item  detect\_lat: latitude of detection in World Geodetic System (WGS) 84 coordinates
            \item  detect\_lon: longitude of detection in WGS84 coordinates
            \item  vessel\_length\_m: length of vessel in meters, where available
            \item  scene\_id: unique xView3 image ID for challenge purposes
            \item  source: source of detection (AIS only, manual only, or both AIS and manual)
            \item  detect\_scene\_row: pixel row of image containing detection
            \item  detect\_scene\_column: pixel column of image containing detection
            \item  detect\_id: unique detection ID
            \item  is\_vessel: True if detection is a vessel, False otherwise, where available
            \item  is\_fishing: True if detection is a fishing vessel, False otherwise, where available
            \item  distance\_from\_shore\_km: distance from shore of detection in kilometers
            \item  confidence: level of confidence for is\_vessel and is\_fishing labels
            \item  top: pixel row of the top left corner of the bounding box, where available
            \item  left: pixel column of the top left corner of the bounding box, where available
            \item  bottom: pixel row of the bottom right corner of the bounding box, where available
            \item  right: pixel column of the bottom right corner of the bounding box, where available
        \end{itemize}
    % \end{enumerate}
    \item \textbf{Is any information missing from individual instances?} \vspace{3pt}
    
    % \begin{enumerate}
        % \item A:
    A subset of objects may be missing:
        \begin{enumerate}
            \item vessel\_length\_m and is\_fishing: these fields are only available where GFW was able to match a given AIS signal to a detection on a SAR image.
            \item is\_vessel: this field is missing if a vessel is matched to an AIS signal but the automated algorithm cannot determine its class.
            \item top, left, bottom, and right: they are only available for manual and both AIS/manual annotations.
        \end{enumerate}
        
    % \end{enumerate}
    \item \textbf{Are there recommended data splits (e.g., training, development/validation, testing)?} \vspace{3pt}
    
    % \begin{enumerate}
        % \item A: 
    Yes. Data is split into train, validation, public, and holdout splits. The \textit{train} and \textit{validation} sets were provided to competitors for training and evaluating their ML models; the \textit{public} set was used for the in-challenge public leaderboard; the \textit{holdout} set was retained for final model performance assessment.
    % \end{enumerate}
    \item \textbf{How was the dataset collected and processed?}  \vspace{3pt}
    
    % \begin{enumerate}
        % \item 
    This question is answered in depth in Section \ref{sec:dataset} of the paper.
    % \end{enumerate}
    \item \textbf{Has the dataset been used for any tasks already?}  \vspace{3pt}
    
    % \begin{enumerate}
        % \item A: 
    The dataset was used for the xView3 Computer Vision Challenge as described in the paper in Section \ref{sec:metric}.
    % \end{enumerate}
    \item \textbf{How will the dataset be distributed? Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?} \vspace{3pt}
    
    % \begin{enumerate}
        % \item A: 
    The dataset is available for download for free, in perpetuity, to anyone who registers for an account at the Challenge website. Note that anyone on the United States Department of State's State Sponsors of Terrorism list (citizens of Syria, North Korea, Iran, and Syria) are unable to download the dataset or participate in the xView3 Computer Vision Challenge.
    % \end{enumerate}
    \item \textbf{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?} \vspace{3pt}
    
    % \begin{enumerate}
        % \item 
    The xView3 dataset contains modified Copernicus Sentinel data (2020). The dataset is distributed under the \href{https://creativecommons.org/licenses/by-nc-sa/4.0/}{Creative Commons Attribution-NonCommercial-ShareAlike 4.0 International} license. Additional terms and conditions on the distribution and use of the dataset and participation in the xView3 Computer Vision Challenge are available on the challenge website at this \href{https://iuu.xview.us/terms-and-conditions}{link}. The authors bear all responsibility for violations of rights.
    % \end{enumerate}
    \item \textbf{Who will be supporting/hosting/maintaining the dataset?} \vspace{3pt}
    
    % \begin{enumerate}
        % \item A: 
    The Defense Innovation Unit, a Department of Defense organization, and its contractors are responsible for maintaining and hosting the dataset.
    % \end{enumerate}
    \item \textbf{How can the owner/curator/manager of the dataset be contacted?} \vspace{3pt}
    % \begin{enumerate}
        % \item A: 
    The managers of the xView3 Computer Vision Challenge and datasets can be contacted at \href{mailto:xview@diu.mil}{xview@diu.mil}.
    % \end{enumerate}
    \item \textbf{Will the dataset be updated?} \vspace{3pt}
    
    % \begin{enumerate}
        % \item A: 
    If the dataset needs to be updated or corrected, it will be further distributed at the Challenge website with a detailed list of errata available from the download portal. All users who have signed up for an account at the challenge website will be updated via an email. Older versions of the dataset will continue to be hosted.
    % \end{enumerate}
\end{enumerate}

==> sec/3_background.tex <==
\section{Background}
\label{sec:background}

\lorem{1}



==> sec/6_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

To allow anyone to easily participate in the xView3 competition, we provide a reference model that incorporates all the modes of data provided. This model is not meant to be a strong baseline, but simply a starting point for competitors built on a reasonable deep learning base. All code for the reference model is provided on \href{https://github.com/DIUx-xView/xview3-reference}{our GitHub repository}.

\subsection{Reference model}
\label{sec:experiments-model}

The reference implementation is a modification on top of the Faster-RCNN architecture \cite{renFasterRCNNRealTime2015}. The model backbone is initialized using pre-trained weights from the ImageNet database. The first layer is replaced by a newly initialized convolutional layer with the appropriate number of input modalities. Note that the classification head is adjusted to handle the number of classes---three in the reference implementation case---used by the implementation.

The model is trained for five epochs on an NVIDIA DGX-1 system with 8x V100 GPUs. Stochastic gradient descent with momentum is used to optimize the model with $\alpha = 5e-3$, momentum of $0.9$, and weight decay of $5e-4$. A step learning rate scheduler is used with step size = $3$ and $\gamma = 0.1$.

\subsection{Results}
\label{sec:experiments-results}
We evaluated our reference model against the \textit{holdout} split. The model scores were as follows: $F1_D = 0.4302$, $F1_S = 0.1293$, $F1_V = 0.6891$, $F1_F = 0.3946$, and $PE_L = 0.0000$ for an aggregate score of $0.1904$.

The reference model made almost no attempt to accurately predict lengths. For every detection centroid a square bounding box of fixed width was created, the diagonal of which was used as the predicted length of the vessel.

==> sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
